A Subjective Dataset for Multi-Screen Video Streaming Applications

In modern-era video streaming systems, videos are streamed and displayed on a wide range of devices. Such devices vary from large-screen UHD and HDTVs to medium-screen Desktop PCs and Laptops to smaller-screen devices such as mobile phones and tablets. It is well known that a video is perceived differently when displayed on different devices. The viewing experience for a particular video on smaller screen devices such as smartphones and tablets, which have high pixel density, will be different with respect to the case where the same video is played on a large screen device such as a TV or PC monitor. Being able to model such relative differences in perception effectively can help in the design of better quality metrics and in the design of more efficient and optimized encoding profiles, leading to lower storage, encoding, and transmission costs. This paper presents a new, open-source dataset consisting of subjective ratings for various encoded video sequences of different resolutions and bitrates (quality) when viewed on three devices of varying screen sizes: TV, Tablet, and Mobile. Along with the subjective scores, an evaluation of some of the most famous and commonly used open-source objective quality metrics is also presented. It is observed that the performance of the metrics varies a lot across different device types, with the recently standardized ITU-T P.1204.3 Model, on average, outperforming their full-reference counterparts. The dataset consisting of the videos, along with their subjective and objective scores, is available freely on Github at https://github.com/NabajeetBarman/Multiscreen-Dataset.

==> Tables/encoding_settings.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|lcclcclcc|}
\hline
\multicolumn{9}{|c|}{\textbf{Low Quality}} \\ 
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Sequence Name}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Resolution}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Bitrate (kbps)}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Sequence   Name}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Resolution}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Bitrate (kbps)}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Sequence   Name}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Resolution}}} & \multirow{2}{*}{\textbf{Bitrate (kbps)}} \\
\multicolumn{1}{|c|}{}                                        & \multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                                         & \multicolumn{1}{c|}{}                                          & \multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                                         & \multicolumn{1}{c|}{}                                          & \multicolumn{1}{c|}{}                                     &                                          \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_L\_540p}}                   & \multicolumn{1}{c|}{540p}                                 & \multicolumn{1}{c|}{11430.91}                                 & \multicolumn{1}{l|}{\textbf{s02\_L\_540p}}                     & \multicolumn{1}{c|}{540p}                                 & \multicolumn{1}{c|}{5153.15}                                  & \multicolumn{1}{l|}{\textbf{s03\_L\_540p}}                     & \multicolumn{1}{c|}{540p}                                 & 900.17                                   \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_L\_720p}}                   & \multicolumn{1}{c|}{720p}                                 & \multicolumn{1}{c|}{14674.72}                                 & \multicolumn{1}{l|}{\textbf{s02\_L\_720p}}                     & \multicolumn{1}{c|}{720p}                                 & \multicolumn{1}{c|}{6623.9}                                   & \multicolumn{1}{l|}{\textbf{s03\_L\_720p}}                     & \multicolumn{1}{c|}{720p}                                 & 1237.73                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_L\_1080p}}                  & \multicolumn{1}{c|}{1080p}                                & \multicolumn{1}{c|}{20881}                                    & \multicolumn{1}{l|}{\textbf{s02\_L\_1080p}}                    & \multicolumn{1}{c|}{1080p}                                & \multicolumn{1}{c|}{9448.75}                                  & \multicolumn{1}{l|}{\textbf{s03\_L\_1080p}}                    & \multicolumn{1}{c|}{1080p}                                & 2179.29                                  \\ \hline
\multicolumn{9}{|c|}{\textbf{Medium   Quality}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_M\_540p}}                   & \multicolumn{1}{c|}{540p}                                 & \multicolumn{1}{c|}{13168.27}                                 & \multicolumn{1}{l|}{\textbf{s02\_M\_540p}}                     & \multicolumn{1}{c|}{540p}                                 & \multicolumn{1}{c|}{6721.47}                                  & \multicolumn{1}{l|}{\textbf{s03\_M\_540p}}                     & \multicolumn{1}{c|}{540p}                                 & 1499.77                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_M\_720p}}                   & \multicolumn{1}{c|}{720p}                                 & \multicolumn{1}{c|}{18962.31}                                 & \multicolumn{1}{l|}{\textbf{s02\_M\_720p}}                     & \multicolumn{1}{c|}{720p}                                 & \multicolumn{1}{c|}{9275.63}                                  & \multicolumn{1}{l|}{\textbf{s03\_M\_720p}}                     & \multicolumn{1}{c|}{720p}                                 & 2084.69                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_M\_1080p}}                  & \multicolumn{1}{c|}{1080p}                                & \multicolumn{1}{c|}{29960.45}                                 & \multicolumn{1}{l|}{\textbf{s02\_M\_1080p}}                    & \multicolumn{1}{c|}{1080p}                                & \multicolumn{1}{c|}{15212.03}                                 & \multicolumn{1}{l|}{\textbf{s03\_M\_1080p}}                    & \multicolumn{1}{c|}{1080p}                                & 3627.35                                  \\ \hline
\multicolumn{9}{|c|}{\textbf{High   Quality}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_H\_540p}}                   & \multicolumn{1}{c|}{540p}                                 & \multicolumn{1}{c|}{16000}                                    & \multicolumn{1}{l|}{\textbf{s02\_H\_540p}}                     & \multicolumn{1}{c|}{540p}                                 & \multicolumn{1}{c|}{16000.02}                                 & \multicolumn{1}{l|}{\textbf{s03\_H\_540p}}                     & \multicolumn{1}{c|}{540p}                                 & 6241.14                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_H\_720p}}                   & \multicolumn{1}{c|}{720p}                                 & \multicolumn{1}{c|}{23360.01}                                 & \multicolumn{1}{l|}{\textbf{s02\_H\_720p}}                     & \multicolumn{1}{c|}{720p}                                 & \multicolumn{1}{c|}{23680.02}                                 & \multicolumn{1}{l|}{\textbf{s03\_H\_720p}}                     & \multicolumn{1}{c|}{720p}                                 & 8487.95                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{s01\_H\_1080p}}                  & \multicolumn{1}{c|}{1080p}                                & \multicolumn{1}{c|}{39945.61}                                 & \multicolumn{1}{l|}{\textbf{s02\_H\_1080p}}                    & \multicolumn{1}{c|}{1080p}                                & \multicolumn{1}{c|}{40019.24}                                 & \multicolumn{1}{l|}{\textbf{s03\_H\_1080p}}                    & \multicolumn{1}{c|}{1080p}                                & 13326.08                                 \\ \hline
\end{tabular}
\end{table}
